Optimal Testing in the Experiment-rich Regime

Motivated by the widespread adoption of large-scale A/B testing in industry, we propose a new experimentation framework for the setting where potential experiments are abundant (i.e., many hypotheses are available to test), and observations are costly; we refer to this as the experiment-rich regime. Such scenarios require the experimenter to internalize the opportunity cost of assigning a sample to a particular experiment. We fully characterize the optimal policy and give an algorithm to compute it. Furthermore, we develop a simple heuristic that also provides intuition for the optimal policy. We use simulations based on real data to compare both the optimal algorithm and the heuristic to other natural alternative experimental design frameworks. In particular, we discuss the paradox of power: high-powered classical tests can lead to highly inefficient sampling in the experiment-rich regime.

==> tex/analysis.tex <==
\section{Analysis}

\subsection{Notation}

For convenience and clarity, we abuse notation and
write $S_n = \sum_{j=1}^n X_j$ for the sum
of outcomes for the current alternative.

\subsection{Conjugate models}

\paragraph{Normal}

Suppose $\mu_i \sim \N(0, \sigma_0^2)$ and $X_i \sim \N(\mu_i, \sigma^2)$
where $X_i$ denotes a an independent draw from alternative $\mu_i$.
Define precision $\tau_0 = 1/\sigma_0$ and $\tau = 1/\sigma$.
Then based on samples $X_1,\ldots,X_n$,
the posterior for $\mu_i$ is given by
\[
    \mu_i \mid X_1,\ldots,X_n \sim
    \N \left(\frac{\sum_{j=1}^n X_j}{n + \gamma},
        \frac{1}{n\tau^2 + \tau_0^2} \right) =
    \N \left(\frac{\sum_{j=1}^n X_j}{n + \gamma},
        \frac{1}{\tau^2(n + \gamma)} \right).
\]
where $\gamma = \tau_0^2 / \tau^2$.
Based on this, we can compute the acceptance region for the current arm,
and find the experimenter can accept the alternative if
\[
    \Phi \left((n\tau^2 + \tau_0^2)(s - \frac{S_n}{n + \gamma}) \right) < \alpha
\]
which, if we define $z_\alpha = \Phi^{-1}(\alpha)$, is equivalent to
\[
    S_n > (n + \gamma)s - \frac{z_\alpha}{\tau} \sqrt{n + \gamma}.
\]
Note that $z_\alpha < 0$ for $\alpha < 0.5$.
It is also trivial to show that
\[
    Y_n = \frac{S_n}{n + \gamma}
\]
is a martingale, with corresponding acceptance boundary
\[
    Y_n > s - \frac{z_\alpha}{\tau\sqrt{n + \gamma}}.
\]

Furthermore, the distribution of $Y_{n+1}$ given $Y_n$ is given by
\[
Y_{n+1} \mid Y_n \sim \N \left(Y_n, \frac{\sigma^2}{(n+\gamma)(n+\gamma+1)} \right)
\]


\paragraph{Beta-Binomial}

Consider the Beta-Binomial setting where
the alternatives are now characterized by a success probability
$p_i \sim \Beta(a, b)$, and samples are Bernoulli draws
$X_t \sim \Bern(p_{i*(t)})$.

It is well known that the posterior given $n$ samples
$X_1, \ldots, X_n$ from alternative $i$ is $\Beta(a + S_n, b + n - S_n)$.



\subsection{Structure of optimal boundary}


\paragraph{Monotonicity}
Let $R_n$ be the rejection region after $n$ samples,
that is, we reject the current alternative if $S_n \in R_n$.
Then we note that $R_n$ must be of the form $(-\infty, r_n)$ for
some $r_n$.

\paragraph{Relation $s$ and $r_n$}
We also note that, contrary to intuition,
there exists cases where $r_n > n s$.
That is, we reject the current alternative, even though the
expected value of the posterior mean is larger than $s$.
Consider the following example in the Normal-Normal model:
Suppose $s = -1$, such that the majority of arms cross the threshold.
If the first sample $X_1$ is sufficiently close to $s$, say $X_1 = -0.9$,
then it is better to reject this alternative in favor of a new alternative
because the new alternative is more likely to be accepted faster.


\paragraph{Avoiding $\mu \approx s$}
It is important for good algorithms to avoid alternatives that are
close to the threshold.
The intuition is that it takes too long to gather enough samples to
decide whether $\mu >s$ or $\mu <s$.
In particular, with probability $\approx c\epsilon$,
$|s - \mu| < \epsilon$, and for such $\mu$, we need approximately
$\frac{1}{\epsilon^2}$ samples. Thus if we do not actively try to avoid
these alternatives, the expected time till acceptance is $\E[T] > \frac{c}{\epsilon}$,
which blows up when $\epsilon \to 0$.

\paragraph{Convergence of boundaries to $s$}
Both the acceptance and rejection boundaries converge to $s$.
That the acceptance region converges follows directly from
the condition $\P(\mu < s) < \alpha$.
For the rejection boundary, we find that if
\[
    \hat X_n \in (s - \frac{z_\alpha}{\tau \sqrt{n+1+\gamma}},
                  s - \frac{z_\alpha}{\tau \sqrt{n + \gamma}})
\]
then, by the martingale property, we expect to accept the next period,
so rejecting cannot be optimal.
As $n \to \infty$, it follows that the rejection boundary converges to $s$
from above.
It is clear that the limit of the optimal rejection boundary cannot be smaller
than $s$.


\subsection{Comparison to fixed horizon test}
It is relatively straightforward to compute the optimal horizon
for maxizing the number of acceptances. We can use this
as a naive benchmark to compare the sequential tests with.

\paragraph{Normal case}
We derive an expression for the time till acceptance in the Normal-Normal case.
Note that after $n$ samples of an alternative, the distribution of $\hat X_n = S_n / (n + \gamma$
is Normal with mean $0$ and variance
\begin{align}
    \var{\bar X_n}
    &= \var{\frac{S_n}{n + \gamma}} \\
    &= \var{\frac{n\mu + \sigma\sum_{i=1}^n Z_i}{n + \gamma}} \\
    &= \frac{ \sigma_0^2 n^2 + \sigma^2 n )}{(n+\gamma)^2}
\end{align}
where $Z_i$ denote independent standard normal random variables.
Thus, the probability to accept an alternative after $n$ observations is
\[
    \P(\text{accept after n observations}) =
    1 - \Phi \left( \frac{n + \gamma }{\sqrt {\sigma_0^2 n^2 + \sigma^2 n} }
                    \left(s - \frac{\sigma z_\alpha }{\sqrt{n + \gamma}} \right)
             \right)
\]
where $z_\alpha = \Phi^{-1}(\alpha)$.
This also makes it easy to compute $\E[T]$ under the fixed threshold policy.

\paragraph{Information and KL-divergence}

Let's analyze the problem in terms of information gain, and the information gap.
Intuitively, the information gain is a measure of the difference in posteriors after
observing another example, while the information gap measures how much
the posterior needs to shift in order to accept the current alternative.

We explore these notions in terms of KL-divergence
\[
    \KL{p}{q} = \int_\Omega \log \frac{p}{q} dp
\]

Note that the KL divergence between $Y \sim \N(\mu_Y, \sigma_Y^2)$ and
$Z \sim \N(\mu_Z, \sigma_Z^2)$ is given by
\[
    \KL{Y}{Z} = \log \frac{\sigma_Z}{\sigma_Y} + \frac{\sigma_Y^2 + (\mu_Y - \mu_Z)^2}{2\sigma_Z^2} - \frac{1}{2}
\]

We define the \emph{information gain} as
\begin{align}
    \textup{Gain}_n
    &= \E_n\left[ \KL{P_{n}}{P_{n+1}} \right]\\
    &= \log \frac{n+\gamma}{n+\gamma+1}
        + \frac{1}{2(n+\gamma)}
        + \frac{(n+\gamma+1) \E[(\frac{S_n}{n+\gamma}  - \frac{S_n + X_{n+1}}{n+\gamma+1})^2]}{2\sigma^2}\\
    &= \log \frac{n+\gamma}{n+\gamma+1}
        + \frac{1}{2(n+\gamma)}
        + \frac{\E_n[(\bar X_n - X_{n+1})^2]}{2\sigma^2(n+\gamma+1)}\\
    &= \log \frac{n+\gamma}{n+\gamma+1}
        + \frac{1}{2(n+\gamma)}
        + \frac{1}{2(n+\gamma+1)}\\
\end{align}

Furthermore, define the \emph{information gap} as the
KL-divergence between the current posterior and a posterior that would accept
the current alternative, i.e.
\[
    \N(s-\frac{\sigma z_\alpha}{\sqrt{n + \gamma}}, \frac{\sigma^2}{n+\gamma})
\]
Since the variances are the same, we find
\[
    \textup{Gap}_n = \frac{(S_n - s(n+\gamma) + \sigma z_a\sqrt{n + \gamma})^2}{2\sigma^2}
\]


\paragraph{Beta-Binomial case}
Let $B(\cdot, \cdot)$ be the Beta function.
Then we find that the probability to accept after $n$ samples in the
fixed horizon setting is

\[
\P(\text{accept after n observations}) =
1-\sum_{k=0}^y \binom{n}{k} \frac{B(a+k, N-k+b)}{B(a, b)}
\]
where $y$ is the minimum number of sampler required to accept after $n$ observations:
\[
    y \in \arg\min_x \P_n(\mu < s \mid S_n = x) < \alpha.
\]



==> tex/discussion.tex <==
\section{Discussion}

Our framework has a few characteristics that are often desirable in practice.
First, dashboards are often used to track the progress of experiments,
e.g. provided by a vendor such as Optimizely used across the web \citep{Johari2017PeekingAA}.
Our framework does not require adjustments for continuous monitoring,
as opposed to many frequentist alternatives.

Traditionally, the null hypothesis testing framework is taught in introductory
statistics classes as a way of conducting experiments. Here, a fixed null hypothesis,
e.g. $H_0: \mu = 0$, is tested against a possibly composite alternative, such as $H_1: \mu > 0$.
In practice, effects are often not precisely zero \citep{mcshane2017abandon}[p.3, p.9], and by collecting
a large enough sample, any such hypothesis would thus be rejected.
Being able to define a specific threshold for a minimum desired effect is often a preferred
way of encoding the problem, as it can be calibrated based on real trade-offs, rather
than an artificial cut-off.

Finally, we think the probabilistic guarantees for discoveries are
easier to understand and interpret by non-experts. The subtleties of frequentist
guarantees make for a much more difficult conversation about understanding of
results. Given that experimentation is becoming more and more ubiquitous,
we believe there is value in simplicity.

% With the advent of the internet economy and the current increase in data and
% computational power, more and more companies use data to guide their decision
% making.  Large companies run thousands of A/B tests every year that aim to
% improve their products \cite{kaufman2017democratizing, google_experiments,
% Kohavi2009OnlineEA, bakshy2014designing}.  In a typical scenario, users to a
% website are randomly assigned either into the control group or treatment group,
% and then metrics are tracked.  An experimenter then uses statistical methods to
% decide whether the treatment group outperforms the control group on these
% metrics.  Often, this takes the form of a hypothesis test, where under the null
% hypothesis, the two alternatives are assumed to lead to the same outcome.


% \subsection{The desiderata of modern experimentation}
% We argue that many modern application of experimentation require the following four
% characteristics
% \begin{enumerate}
%     \itemsep0em
%     \item Tests are sequential and allow for peeking.
%     \item There are many alternatives that can be tested, which leads
%         to an opportunity cost for each observation.
%     \item Experimenters care about guarantees of the effect size.
%     \item Results need to be intuitive and understandable to non-experts
% \end{enumerate}
% We expand on each of these in the following paragraphs.

% \paragraph{Sequential testing}
% In traditional hypothesis testing, as taught in any introductory class on
% statistics, the experimenter first posits a hypothesis, then gathers all the
% data, and finally makes a decision based on a test statistic.  However, in
% comtemporary applications, such as in A/B testing, it is often possible, even
% trivial, to acquire data sequentially and monitor tests sequentially.  On one
% hand, this requires extra care from statisticians to ensure that the testing
% procedures are correct under continuous monitoring, and indeed there has been a
% lot of work on this \citep{lai1988nearly, lai1997optimal,
% siegmund2013sequential, Johari2017PeekingAA} On the other hand, this allows
% procedures to be adaptive to the difficulty of the testing problem at hand, and
% therefore can be much more efficient.  For example, when the effect size is
% large, only few samples are needed to detect such deviation, while when the
% effect size is small, many more samples are needed before conclusions can be
% drawn from data.  If the sample size is fixed ahead of time, the experimenter
% might thus collect too many or too few samples.  A sequential tests can stop
% early when the effect size is large, and continue sampling when the effect size
% turns out to be small.

% \paragraph{Opportunity costs}
% In (frequentist) hypothesis testing, there are two types of errors: first a
% test can falsely reject the null hypothesis even though it is true (Type I
% error), or it can falsely fail to reject the null hypothesis (Type II error).
% These two types of errors are in conflict with each other.  E.g. by always
% rejecting a test, the experimenter protects herself against Type II errors, but
% has high Type I error rate.  Thus to balance these two error rates, the
% experimenter constrains the Type I error to a fixed significance $\alpha$.  A
% good test then is one that, given control of the Type I error rate, has high
% \emph{power}, which is loosely defined as the probability of correctly
% rejecting the null hypothesis.

% However, when there are many potential alternatives to test, and
% we use a sequential testing procedure, the focus on power is misguided, because
% it fails to account for the opportunity cost of other alternatives.  In
% particular, suppose that the effect size of the current alternative we are
% testing is small, then it takes a lot of observations to tease this apart.  But
% these observations could have been used to test alternatives that are more
% promising.  A better testing procedure ignores these smaller effects and ignores
% power as a metric. Intsead, it aims to find larger effects.

% \paragraph{Effect size}
% Traditionally, the experimenter specifies a null hypothesis,
% e.g. $H_0: \theta = 0$ and an
% alternative hypothesis, $H_1: \theta \neq 0$.
% We know that in many applications, as we increase the number of samples,
% the experimenter would always reject the null hypothesis;
% it is unlikely that the parameter is \emph{exactly} zero and with enough data,
% any small deviation will eventually be detected with enough samples.
% But such tiny effects are irrelevant to the experimenter.
% That is, the effect size is relevant and this should be captured by
% the testing framework.

% In practice, there is usually also a cost involved in implementing a particular
% alternative. Thus, no energy should be wasted on making changes that hardly
% make a difference.  Instead, it makes more sense for the experimenter to
% specify a desired minimum effect size. One could encode this in the null
% hypothesis, e.g. specify $H_0: \theta = \Delta$ in our toy example above, where
% $\Delta$ is the desired effect.
% But this blurs the lines between statistical assumptions and goals.
% We thus advocate for a more direct approach.

% \paragraph{Interpretation}
% In most cases, results from A/B tests need to be communicated with non-experts,
% such as business partners which lack the necessary statistical background.
% Whether you are a proponent or opponent \citep{carver1978case,
% mcshane2017abandon} of p-values, we all agree that interpretation of the
% frequentist approach to hypothesis testing is challenging for people less
% versed in probability \citep{Goodman2008ADD}.

% Furthermore, we have to deal with multiple tests, for example by providing
% FDR control, in a sequential fashion, say using alpha-investing.  This is
% challenging even for experts, and thus we should be willing to pay a premium
% for simple methods that are easy to interpret and explain.


==> tex/misc.tex <==

    \appendix
    % Other material:
    \textbf{This is just for reference, will be removed}

    \input{tex/analysis}

    \section{Multiple comparisons / MAB}

    What if an experiment involves multiple arms / options?

    \section{Alternative strategies}
        Fixed horizon

        Frequentist + adjusted p-values + alpha-investing

        Thompson sampling

        Simple Bayesian strategy: Select new arm if $\P(\mu_{i+1} > s) > \P(\mu_i > s)$:
        a new arm has higher probability of being larger than $s$ than the current arm,
        which means we need to keep making progress to outpace the reduction
        in uncertainty about $\mu_i$.
        This seems to be rather slow when $\mu_i \approx s$.

    \section{Incorporating cost of reset}

    Implementing a new test can be costly, so add cost $c$ to the
    reject action. This should be easy to incorporate.

    \section{Simulations}

    \section{Discussion}

    \subsection{Downsides}

    Estimation; estimates for effect size are wrong.
    Well known downside of sequential tests \cite[Chapters 3 and 4]{siegmund2013sequential}

    Arguably, this is not such a big deal; if there is a positive effect,
    can run the experiment longer to get a good estimate. The real
    key is to reject fast when there is no effect.



